Accelerating Nesterov's Method for Strongly Convex Functions with Lipschitz Gradient

We modify Nesterov's constant step gradient method for strongly convex functions with Lipschitz continuous gradient described in Nesterov's book. Nesterov shows that $f(x_k) - f^* \leq L \prod_{i=1}^k (1 - \alpha_k) \| x_0 - x^* \|_2^2$ with $\alpha_k = \sqrt{\rho}$ for all $k$, where $L$ is the Lipschitz gradient constant and $\rho$ is the reciprocal condition number of $f(x)$. Hence the convergence rate is $1-\sqrt{\rho}$. In this work, we try to accelerate Nesterov's method by adaptively searching for an $\alpha_k > \sqrt{\rho}$ at each iteration. The proposed method evaluates the gradient function at most twice per iteration and has some extra Level 1 BLAS operations. Theoretically, in the worst case, it takes the same number of iterations as Nesterov's method does but doubles the gradient calls. However, in practice, the proposed method effectively accelerates the speed of convergence for many problems including a smoothed basis pursuit denoising problem.

==> notations.tex <==

\section*{Notations {\color{red} [for reference only, not in final version]}}
\label{sec:notations}

\begin{itemize}
\item $f$, a function from $S_{\mu,L}^{1,1}(\mathbb{R}^n)$
\item $L$, Lipschitz constant of $f'$
\item $\mu$, strong convexity parameter of $f$
\item $\kappa = L/\mu$, condition number of $f$
\item $\rho = 1/\kappa$, reciprocal condition number of $f$
\item $\alpha_0 = \sqrt{\rho}$, Nesterov's choice of $\alpha_k$ each $k$
\item $\alpha_k$, parameter controlling the rate of decrease at the $k$-th iteration
\item $x_k$, $v_k$, and $y_k$, points
\item $\tilde{\alpha}_k$, $\tilde{x}_k$, $\tilde{v}_k$, and $\tilde{y}_k$, trial points
\item $D_k = = \mu^2 \| x_k - v_k \|^2 / \| f'(y_{k-1}) \|^2$
\item $\eta_k( \alpha ) = \alpha^3 + ( 1 + D_k ) \alpha^2 - ( \rho + D_k ) \alpha - \rho$
\item $\beta_k$, the positive local minimum of $\eta_k$
\item $\gamma_k$, the positive root of $\eta_k$
\item $\mathcal{N}_{\mu,L}$, Nesterov's method for functions from $S_{\mu,L}^{1,1}$
\item $\mathcal{N}_{L}$, Nesterov's method for functions from $S_{L}^1$
\item $\mathcal{N}_{\mu,L}^\alpha$, Nesterov's method with adaptive $\alpha_k$
\end{itemize}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "acc_nesterov"
%%% End: 

